The geometry of efficient codes: how rate-distortion trade-offs distort the latent representations of generative models

Living organisms rely on internal models of the world to act adaptively. These models, because of resource limitations, cannot encode every detail and hence need to compress information. From a cognitive standpoint, information compression can manifest as a distortion of latent representations, resulting in the emergence of representations that may not accurately reflect the external world or its geometry. Rate-distortion theory formalizes the optimal way to compress information while minimizing such distortions, by considering factors such as capacity limitations, the frequency and the utility of stimuli. However, while this theory explains why the above factors distort latent representations, it does not specify which specific distortions they produce. To address this question, here we investigate how rate-distortion trade-offs shape the latent representations of images in generative models, specifically Beta Variational Autoencoders ($\beta$-VAEs), under varying constraints of model capacity, data distributions, and task objectives. By systematically exploring these factors, we identify three primary distortions in latent representations: prototypization, specialization, and orthogonalization. These distortions emerge as signatures of information compression, reflecting the model's adaptation to capacity limitations, data imbalances, and task demands. Additionally, our findings demonstrate that these distortions can coexist, giving rise to a rich landscape of latent spaces, whose geometry could differ significantly across generative models subject to different constraints. Our findings contribute to explain how the normative constraints of rate-distortion theory shape the geometry of latent representations of generative models of artificial systems and living organisms.

==> src/figures.tex <==
% \includegraphics[width=.2\columnwidth]{imgs/img_clf0.png}

\begin{comment}
\begin{figure}
\centering
\begin{minipage}{.47\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{assets/eucl_emb_clf0.pdf}
  \caption{figure}{Example of reconstructions on the Italian dataset. The test input sample is in blue and then repeated in orange, reconstruction is in green.}
  \label{fig:third_recs}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}{.47\textwidth}
  \centering
  \includegraphics[width=\columnwidth]{assets/eucl_emb_clf1.pdf}
  \caption{figure}{Proposed convolutional variational attention mechanism.}
  \label{fig:Convolutional Variational Self-Attention}
\end{minipage}
\end{figure}    
\end{comment}



\begin{comment}
    
\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/intro1.pdf}
\caption{rdt framework and bvae architecture}
\label{fig:intro1}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/intro2.pdf}
\caption{probability vs capacity. Bias on lower corridor: it appears on the left (pixel $\leq 6$) 10 times more often than on the right}
\label{fig:intro2}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/intro3.pdf}
\caption{relevance vs capacity. 2 inputs: in a case they are not relevant (they have same label) for task2 (and thus they collapse in the same image when the capacity is low), in the other case they are relevant (different labels) for task3.}
\label{fig:intro3}
\end{center}
\end{figure}

\end{comment}




\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/clf/task0.pdf}
\caption{task0 \textcolor{blue}{decidere se chiamarla sparsification}}
\label{fig:task0}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/clf/task1.pdf}
\caption{
Task1. 
\textbf{(A)} 2D embedding of the 5D latent representation of test images under the baseline model at high capacity. 
\textbf{(B)} 5 matrices representing the activation patterns of the 5 neurons of the latent representation of the model in panel A. Each matrix is computed as in sec. \ref{sec:neuron_activity}. 
\textbf{(C)} 2D embedding of the 5D latent representation of test images under the hybrid model trained on task 1 at high capacity. 
\textbf{(D)} 5 matrices representing the activation patterns of the 5 neurons of the latent representation of the model in panel C. 
\textbf{(F)} 2D embedding of the 5D latent representation of test images under the baseline model at low capacity. 
\textbf{(G)} 5 matrices representing the activation patterns of the 5 neurons of the latent representation of the model in panel F. 
\textbf{(H)} 2D embedding of the 5D latent representation of test images under the hybrid model trained on task 1 at low capacity. 
\textbf{(I)} 5 matrices representing the activation patterns of the 5 neurons of the latent representation of the model in panel H.
}
\label{fig:task1}
\end{center}
\end{figure}



\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/clf/task3.pdf}
\caption{task3}
\label{fig:task3}
\end{center}
\end{figure}



\begin{comment}

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/eucl_emb_clf0.pdf}
\caption{Results of experiment S1E4. The hybrid network is assigned a binary classification task: we labeled with $1$ the images in which the corridors are aligned ($x_L = x_U$) and with $0$ all the other images. Plots A and C contain the latent representation learned by the baseline $\beta$-VAE when trained at high and low capacity respectively; see section \ref{sec:baseline_net} for the description of the latent space. Plots B and D contain the latent representation learned by the hybrid network when trained at high and low capacity respectively. At high capacity the representation still has a square-like shape as in A but points belonging to class $1$ have been remapped at the vertices of the square while at low capacity this shape is completely lost an all the datapoints collapse into two clusters corresponding to the two classes in the dataset.}
\label{fig:clf0}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/eucl_emb_clf1.pdf}
\caption{Results of experiment S1E3. The hybrid network is assigned a binary classification task: we labeled with $1$ the images in which the corridors are aligned ($x_L = x_U$) and with $0$ all the other images. Plots A and C contain the latent representation learned by the baseline $\beta$-VAE when trained at high and low capacity respectively; see section \ref{sec:baseline_net} for the description of the latent space. Plots B and D contain the latent representation learned by the hybrid network when trained at high and low capacity respectively. At high capacity the representation still has a square-like shape as in A and the distortion translates into a better separation of the datapoints belonging to different classes while at low capacity this shape is completely lost an all the datapoints collapse into few clusters corresponding to the few classes the net is able to distinguish with the available capacity.}
\label{fig:clf1}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/eucl_emb_clf2.pdf}
\caption{Results of experiment S1E2. The hybrid network is assigned a binary classification task: we labeled with $1$ the images in which $x_U \leq x_L$ and with $0$ all the other images. Plots A and C contain the latent representation learned by the baseline $\beta$-VAE when trained at high and low capacity respectively; see section \ref{sec:baseline_net} for the description of the latent space. Plots B and D contain the latent representation learned by the hybrid network when trained at high and low capacity respectively. At high capacity the representation still has a square-like shape as in A and the distortion translates into a better separation of the datapoints belonging to different classes while at low capacity this shape is completely lost an all the datapoints collapse into two clusters corresponding to the two classes in the dataset.}
\label{fig:clf2}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/eucl_emb_clf3.pdf}
\caption{Results of experiment S1E1. The hybrid network is assigned a binary classification task: we labeled with $1$ the images in which $x_U <6$ (regardless of the value of $x_L$) OR $( x_U \geq 6$ AND $x_L \geq 6 )$ and with $0$ all the other images. Plots A and C contain the latent representation learned by the baseline $\beta$-VAE when trained at high and low capacity respectively; see section \ref{sec:baseline_net} for the description of the latent space. Plots B and D contain the latent representation learned by the hybrid network when trained at high and low capacity respectively. At high capacity the representation still has a square-like shape as in A and the distortion translates into a better separation of the datapoints belonging to different classes while at low capacity this shape is completely lost an all the datapoints collapse into two clusters corresponding to the two classes in the dataset.} 
\label{fig:clf3}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/eucl_emb_all_disent.pdf}
\caption{Results of experiment S2E1. The hybrid has to solve all the 4 classification tasks of part 1 simultaneously. To read the images easier, we used the same colors as in E1S1. Plots A and C contain the latent representation learned by the baseline $\beta$-VAE when trained at high and low capacity respectively; see section \ref{sec:baseline_net} for the description of the latent space. Plots B and D contain the latent representation learned by the hybrid network when trained at high and low capacity respectively. At high capacity the network learns a representation that is both disentangled and helpful to solve all the classification tasks. In fact, the 25 classes of experiment S1E4 have been clearly separated in the new representation. Furthermore, by looking closer at plot B, it is possible to observe that images that belong to the same class in task S1E4, like (6,0) and (5,1), are further separated to solve the other classification tasks (in this case the two images are separated because they belongs to 2 different classes in S1E1). At low capacity, {\color{blue} forse meglio mettere questo plot nei supplementary visto che il training e' diverso da tutti gli altri ed il classificatore parte dopo}}
\label{fig:all_clf_disent}
\end{center}
\end{figure}







\end{comment}

\begin{comment}
\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/eucl_emb_all_ent.pdf}
\caption{4 classifiers, activated since the beginning (actually, to make the net learn the task0 I had to give a larger weigth to the corresponding loss)}
\label{fig:all_clf_ent}
\end{center}
\end{figure}    
\end{comment}


\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{assets/rec_samples.pdf}
\caption{Reconstruction samples}
\label{fig:rec_samples}
\end{center}
\end{figure}


==> src/methods-old.tex <==
\section{Methods}

\textcolor{red}{inserire immagini del dataset, del vae base e del vae+clf}
\\

\textcolor{red}{trovare esempi di task in cui devi ricordare informazioni su percorsi ecc}
\\

\textcolor{red}{nel task sbilanciato, provare a trovare una misura di quanto l'input e' lontano dalla media della distribuzione appresa - sorpresa, KL}
\\

In our experiments, we examined the distortions arising in the representation learned by a Beta Variational Autoencoder ($\beta$-VAE) \cite{bvae_2017} under different training conditions. 
Our experiments can be divided into two sets: the first set involves studying the distortions induced by statistically biased training sets by comparing the representations learned by the same neural network, first trained on an unbiased dataset, and then trained on a biased one. 
The second set involves studying the distortions induced by a given classification task assigned to the network. 
To do this, we compared the representation learned by the network when the only objective was to reconstruct input images against the representation learned when the objective was augmented with a classification task. 
In both sets of experiments, we trained multiple networks by varying their encoding capacity to study how this impacts on the magnitude of distortions.
\\

\noindent \textbf{Dataset.} The dataset we generated consists of $n=500000$ black and white 13x13 images containing 2 vertical noisy corridors, one in the upper part of the image and the other one in lower part. 
In each image, the upper and lower sections are separated by an horizontal line with width 1 pixel. 
The positions of the upper corridor ($x_{UC}$) and of the lower corridor ($x_{LC}$) are two integers that represent the two factors of variation of the dataset, since they can slide horizontally from pixel 0 to pixel 12 across images. 
Each pixel of the image was obtained as an independent sample from a Bernoulli distribution $f(g(x;\mu, \sigma))$, where $g(x;\mu, \sigma)$ is a Gaussian probability density function with standard deviation $\sigma=1.2$ and mean $\mu=x_{UC}$ if the pixel is in the upper half of the image, $\mu=x_{LC}$ otherwise.
\\

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{sample_image_13x13}
\caption{Example of an image in the dataset. Here the upper corridor is in horizontal position $x_{UC}=7$, while the lower is in $x_{LC}=3.$}
\end{figure}


\noindent \textbf{Models.} The base neural network architecture we used in our experiments is the Beta Variational Autoencoder ($\beta$-VAE) . 
The encoder block consists of 3 convolutional layer, each followed by a leaky ReLU activation. Similarly, the decoder block consists of 3 transposed convolutional layers, also followed by a leaky ReLU activation function, except for the last layer having a sigmoid activation function to output grayscale images. We fixed the dimension of the latent rapresentation to $5$ and we trained the network by increasing the encoding capacity $C$ from $0$ to a target value $C_{max}$ during training \cite{bvae_2018}. 

In the second set of experiments, we slightly modified the neural network by embedding a classifier into the $\beta$-VAE architecture. 
The classifier takes as input the $5$-dimensional latent vector the encoder associates to each image and its loss function is added to the $\beta$-VAE's loss. 
Thus, by jointly training the classifier and the $\beta$-VAE, the new architecture learns how to solve a given classification task while still learning to reconstruct the input images. 
This joint training procedure allows us to study the distortion induced by the classification task on the latent representation learnt by the $\beta$-VAE. 
Depending on the specific task, the classifier can be linear or non-linear. The linear classifier is a feedforward neural network with no activations and a single hidden layer with 1024 units. The non-linear classifier is a feedforward neural network with leaky ReLU activations and a single hidden layer with 1500 units.
\\

\noindent \textbf{Comparing latent representations.} Our goal is to compare the geometry of the latent space learned by a network A with the that learned by an other network B. 
Since in our experiments the latent space is 5-dimensional, we reduce its dimensionality through Multidimensional Scaling (MDS) \cite{borg2005modern} to obtain 2D visualizations of the structure of the latent space. 
MDS requires as input a matrix representing dissimilarities between pairs of images. For a given network A, we obtain the dissimilarity matrix by computing the \textcolor{red}{euclidean distance or correlation?} between the 5-dimensional vectors associated to the each image by the encoder block of the network. Once this is done, we compute the 2D embedding of the latent space through MDS. We do the same for the network B and we qualitatively compare the two 2D plots of the embeddings.
\\

\noindent \textbf{Experiments, part 1.} In order to examine the distortions induced by statistically biased training sets on the representation learned by a $\beta$-VAE we run two experiments and we call them S1E1 and S1E2 respectively. 
In S1E1 we trained the network on an unbalanced dataset in which the images with the lower corridor on the left appears 10 times more often than images with the lower corridor on the right. Let $x_L$ be the pixel at which the lower corridor is centered, then "lower corridor on the left" means that $x_L \leq 6$, where $x_L \in \{0,1,\ldots,12\}$. 
In S1E2 we trained the network on an unbalanced dataset in which the images having the two corridors aligned ($x_L = x_U$) appears 10 times more often than images with non-aligned corridors. 
In both S1E1 and S1E2, we repeated the training for different values of encoding capacity $C_{max} \in \{0.3, 1, 3, 6, 10\}$ nats. 
We compared the representation learned by the networks in S1E1 and S1E2 against the one learned by the same networks trained on a balanced dataset. The results are shown in (fig here). (Comment the result here)
\\

\noindent \textbf{Experiments, part 2.}  In order to examine the distortions induced by a given classification task assigned to the network on the representation learned by a $\beta$-VAE we run four experiments, each corresponding to a different classification task, and we call them S2E1, S2E2, S2E3 and S2E4 respectively. 
Therefore, in all experiments, we train the hybrid network described above ($\beta$-VAE + classifier) in a supervised manner on a dataset containing always the same images that are relabel from experiments to experiments according to the specific classification task. 
In all the experiments the classifier is linear, except in S1E1 where we adopt the non-linear classifier described before. 
As before, in each experiment, we repeated the training for different values of encoding capacity $C_{max} \in \{0.3, 1, 3, 6, 10\}$ nats. 
The latent representations learned by the hybrid network in S2E1,..., S2E4 are compared against the representation learned by the usual $\beta$-VAE on the same dataset.

In S2E1, ... 

In S2E2, the network is assigned a binary classification task. We labeled with $1$ the images in which the corridors are aligned ($x_L = x_U$) and with $0$ all the other images. (Comment the result here)

In S2E3, the network is assigned a binary classification task. We labeled with $1$ the images in which $x_U \leq x_L$ and with $0$ all the other images.(Comment the result here)

In S2E4, the network is assigned a binary classification task. We labeled with $1$ the images in which $x_U <6$ OR $( x_U \geq 6$ AND $x_L \geq 6 )$ and with $0$ all the other images. (Comment the result here)
\\

%trained a Beta Variational Autoencoder ($\beta$-VAE) \cite{bvae_2017} on a synthetic dataset 

\begin{figure}
\begin{center}
\includegraphics[width=.4\linewidth]{imgs/clf_bias/task0/eucl_t0_base_high_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/clf_bias/task0/eucl_t0_distorted_high_emb.png}
\\%[\baselineskip]% adds vertical line spacing
\includegraphics[width=.4\linewidth]{imgs/clf_bias/task0/eucl_t0_base_low_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/clf_bias/task0/eucl_t0_distorted_low_emb.png}
\caption{classification task0}
\label{fig:enter-label}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=.4\linewidth]{imgs/clf_bias/task1/eucl_t1_base_high_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/clf_bias/task1/eucl_t1_distorted_high_emb.png}
\\%[\baselineskip]% adds vertical line spacing
\includegraphics[width=.4\linewidth]{imgs/clf_bias/task1/eucl_t1_base_low_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/clf_bias/task1/eucl_t1_distorted_low_emb.png}
\caption{classification task1}
\label{fig:enter-label}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=.24\linewidth]{imgs/clf_bias/task1/eucl_t1_base_high_emb.png}
\includegraphics[width=.24\linewidth]{imgs/clf_bias/task1/eucl_t1_distorted_high_emb.png}
%[\baselineskip]% adds vertical line spacing
\includegraphics[width=.24\linewidth]{imgs/clf_bias/task1/eucl_t1_base_low_emb.png}
\includegraphics[width=.24\linewidth]{imgs/clf_bias/task1/eucl_t1_distorted_low_emb.png}
\caption{classification task1}
\label{fig:enter-label2}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=.4\linewidth]{imgs/clf_bias/task2/eucl_t2_base_high_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/clf_bias/task2/eucl_t2_distorted_high_emb.png}
\\%[\baselineskip]% adds vertical line spacing
\includegraphics[width=.4\linewidth]{imgs/clf_bias/task2/eucl_t2_base_low_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/clf_bias/task2/eucl_t2_distorted_low_emb.png}
\caption{classification task2}
\label{fig:enter-label}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=.4\linewidth]{imgs/clf_bias/task3/eucl_t3_base_high_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/clf_bias/task3/eucl_t3_distorted_high_emb.png}
\\%[\baselineskip]% adds vertical line spacing
\includegraphics[width=.4\linewidth]{imgs/clf_bias/task3/eucl_t3_base_low_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/clf_bias/task3/eucl_t3_distorted_low_emb.png}
\caption{classification task3}
\label{fig:enter-label}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=.4\linewidth]{imgs/stat_bias/AlignBias/eucl_ts_base_high_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/stat_bias/AlignBias/eucl_ts_distorted_high_emb.png}
\\%[\baselineskip]% adds vertical line spacing
\includegraphics[width=.4\linewidth]{imgs/stat_bias/AlignBias/eucl_ts_base_low_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/stat_bias/AlignBias/eucl_ts_distorted_low_emb.png}
\caption{dataset bias: aligned corridors}
\label{fig:enter-label}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=.4\linewidth]{imgs/stat_bias/BottomBias/eucl_ts_base_high_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/stat_bias/BottomBias/eucl_ts_distorted_high_emb.png}
\\%[\baselineskip]% adds vertical line spacing
\includegraphics[width=.4\linewidth]{imgs/stat_bias/BottomBias/eucl_ts_base_low_emb.png}\quad\includegraphics[width=.4\linewidth]{imgs/stat_bias/BottomBias/eucl_ts_distorted_low_emb.png}
\caption{dataset bias: lower corridor}
\label{fig:enter-label}
\end{center}
\end{figure}
